Multi-band programmable gain Raman amplifier

Optical communication systems, operating in C-band, are reaching their theoretically achievable capacity limits. An attractive and economically viable solution to satisfy the future data rate demands is to employ the transmission across the full low-loss spectrum encompassing O, E, S, C and L band of the single mode fibers (SMF). Utilizing all five bands offers a bandwidth of up to $\sim$53.5THz (365nm) with loss below 0.4dB/km. A key component in realizing multi-band optical communication systems is the optical amplifier. Apart from having an ultra-wide gain profile, the ability of providing arbitrary gain profiles, in a controlled way, will become an essential feature. The latter will allow for signal power spectrum shaping which has a broad range of applications such as the maximization of the achievable information rate X distance product, the elimination of static and lossy gain flattening filters (GFF) enabling a power efficient system design, and the gain equalization of optical frequency combs. In this paper, we experimentally demonstrate a multi-band (S+C+L) programmable gain optical amplifier using only Raman effects and machine learning. The amplifier achieves >1000 programmable gain profiles within the range from 3.5 to 30 dB, in an ultra-fast way and a very low maximum error of 1.6e-2 dB/THz over an ultra-wide bandwidth of 17.6-THz (140.7-nm).

==> style.tex <==
\usepackage[lmargin=2cm, rmargin=2cm, tmargin=2cm, bmargin=2cm]{geometry}
\usepackage{mathptmx,amsmath}
\usepackage{amssymb}
\usepackage[pdftex]{graphicx}
\usepackage[caption=false,font=footnotesize]{subfig}
\usepackage[T1]{fontenc}
%\usepackage{enumerate}
\usepackage{hyperref}
\usepackage{indentfirst}    %indent first paragraph of each section
\usepackage{soul}
\usepackage{xspace}
\usepackage{xcolor}
%\usepackage[hyphens]{url}
\usepackage{quoting}

\pagestyle{plain}
\pagenumbering{arabic}
\renewcommand{\arraystretch}{1.3}

\hyphenpenalty=50000
\tolerance=10000

\hypersetup
{
    pdftitle={Response To Reviewers Comments},
    pdfauthor={},
    colorlinks=true,
    linkcolor=black,
    citecolor=black,
    urlcolor=blue,
    pdfview=Fit,
    pdfpagemode=UseNone
}
\graphicspath{{./figures/}}
\renewcommand{\captionsize}{\footnotesize}
\definecolor{myblue}{rgb}{0.0,0.25,0.50}
\definecolor{myred}{rgb}{0.64,0.08,0.18}

% \newcommand{\revComment}[1]{\color{myblue}``\textit{\textbf{#1}}''}
\newcommand{\revComment}[1]{\color{myblue}``\emph{#1}''}
\newcommand{\authorResponse}{\color{black}\textbf{Authors' Response: }}
\newcommand{\reference}[1]{\vspace{0.1cm}\noindent\small\color{black}#1\color{black}\normalsize\vspace{0.1cm}}
\newcommand{\paperModification}[1]{\vspace{0.1cm}\noindent\color{red}#1\color{black}\normalsize\vspace{0.1cm}}
